Progress, Justness and Fairness

Fairness assumptions are a valuable tool when reasoning about systems. In this paper, we classify several fairness properties found in the literature and argue that most of them are too restrictive for many applications. As an alternative we introduce the concept of justness.

==> acmart-preload-hook.tex <==
\RequirePackage[bookmarksnumbered,unicode,hyperfootnotes=false,hypertexnames=false]{hyperref}

